A Variant of Earley Deduction With Partial Evaluation

We present an algorithm for query evaluation given a logic program consisting of function-free Datalog rules. It is based on Earley Deduction [4, 6] and uses a partial evaluation similar to the one we devel oped for our SLDMagic method [1]. With this, finite automata modeling the evaluation of given queries are generated. In certain cases, the new method is more efficient than SLDMagic and the standard Magic Set method since it can process several deduction steps as one.

==> defWLP12.tex <==
\makeatletter
\def\define#1{\@ifnextchar [{\@MYargdef#1}{\@MYargdef#1[0]}}

\def\@MYargdef#1[#2]#3{\@ifdefinable #1{\@MYreargdef#1[#2]{#3}}}

\def\redefine#1{\edef\@tempa{\expandafter\@cdr\string 
  #1\@nil}\@ifundefined{\@tempa}{\@latexerr{\string#1\space undefined}\@ehc
    }{}\@ifnextchar [{\@MYreargdef#1}{\@MYreargdef#1[0]}}

\catcode`\?=11\relax
\def\@MYreargdef#1[#2]#3{\@tempcnta#2\relax\let#1\relax
\edef\@tempa{\def#1}\@tempcntb \@ne
\let\@?@?\relax\@whilenum\@tempcnta>0
\do{\edef\@tempa{\@tempa\@?@?\the\@tempcntb}\advance\@tempcntb \@ne \advance
\@tempcnta \m@ne}\let\@?@?##\@tempa{#3}}
\catcode`\?=12\relax
\makeatother

\define{\doSubst}[2]{#2\,#1}
\define{\idFont}{\sf}
\define{\id}[1]{{\idFont #1}}
\define{\Rule}{\id{R}}
\define{\fact}{\id{F}}
\define{\prog}{\mathcal{P}}
\define{\db}{\mathcal{D}}
\define{\state}{\mathcal{S}}
\define{\answerPred}{\id{answer}}
\define{\andUntil}{\wedge \cdots \wedge}
\define{\until}{, \ldots, }
\define{\union}{\cup}
\define{\lineno}[1]{\hbox to 1.6em{\hfil$\lbrack#1\rbrack$}}
\define{\lineref}[1]{$\lbrack#1\rbrack$}
\define{\comment}[1]{//\textnormal{#1}}
\define{\path}{\id{path}}
\define{\edge}{\id{edge}}
\define{\varA}{\id{X}_0}
\define{\varB}{\id{X}_1}
\define{\varC}{\id{X}_2}
\define{\litA}{\id{A}}
\define{\litB}{\id{B}}
\define{\litC}{\id{C}}
\define{\lif}{\leftarrow}
\define{\subst}{\theta}

